The simplest derivation of the Lorentz transformation

Starting from the well-known light-clock thought experiment to derive time dilation and length contraction, it is shown that finding the Lorentz Transformation requires nothing more than the most trivial vector addition formula. The form which is obtaine for the L.T. allows an easy derivation of the velocity and acceleration transformations which are also given.

==> dico.tex <==
\newcommand{\bm}{\boldmath}
\newcommand{\ebm}{\unboldmath}
\newcommand{\bee}{\begin{enumerate}}
\newcommand{\bei}{\begin{itemize}}
\newcommand{\beq}{\begin{eqnarray*}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\ene}{\end{enumerate}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\eeq}{\end{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\vide}{{\rm O}\!\!\!\!\slash }
\newcommand{\evt}{\'ev\'enement }
\newcommand{\evts}{\'ev\'enements }
\newcommand{\prob}{probabilit\'e }
\newcommand{\va}{variable al\'eatoire }
\newcommand{\vas}{variables al\'eatoires }
\newcommand{\Vas}{Variables al\'eatoires }
\newcommand{\de}{$\delta\;$}
\newcommand{\indpt}{ ind\'ependants }
\newcommand{\indpte}{ ind\'ependantes }
\newcommand{\demi}[1]{$\frac{#1}{2}$}
\newcommand{\demipi}[1]{$\frac{#1}{2\pi}$}
\newcommand{\Demi}[1]{\frac{#1}{2}}
\newcommand{\Demipi}[1]{\frac{#1}{2\pi}}
\newcommand{\sft}[2]{\section{#1}\footnote{#2}}
\newcommand{\ssft}[2]{\subsection{#1 \footnote {#2}}}
\newcommand{\sssft}[2]{\subsubsection{#1}\footnote{#2}}
\newcommand{\er}{\raisebox{3pt}{{\small er}}}
\newcommand{\eme}{\raisebox{3pt}{{\small \`eme}}}
\newcommand{\Om}{$\Omega$ }
\newcommand{\om}{$\omega$ }
\newcommand{\exo}{$\Rightarrow$ }
\newcommand{\reel}{${\Bbb R}$ }
\newcommand{\emat}{ esp\'erance math\'ematique }
\newcommand{\var}{variance }

